Neutralizing Backdoors through Information Conflicts for Large Language Models

Large language models (LLMs) have seen significant advancements, achieving superior performance in various Natural Language Processing (NLP) tasks, from understanding to reasoning. However, they remain vulnerable to backdoor attacks, where models behave normally for standard queries but generate harmful responses or unintended output when specific triggers are activated. Existing backdoor defenses often suffer from drawbacks that they either focus on detection without removal, rely on rigid assumptions about trigger properties, or prove to be ineffective against advanced attacks like multi-trigger backdoors. In this paper, we present a novel method to eliminate backdoor behaviors from LLMs through the construction of information conflicts using both internal and external mechanisms. Internally, we leverage a lightweight dataset to train a conflict model, which is then merged with the backdoored model to neutralize malicious behaviors by embedding contradictory information within the model's parametric memory. Externally, we incorporate convincing contradictory evidence into the prompt to challenge the model's internal backdoor knowledge. Experimental results on classification and conversational tasks across 4 widely used LLMs demonstrate that our method outperforms 8 state-of-the-art backdoor defense baselines. We can reduce the attack success rate of advanced backdoor attacks by up to 98% while maintaining over 90% clean data accuracy. Furthermore, our method has proven to be robust against adaptive backdoor attacks. The code will be open-sourced upon publication.

==> algo/main-algorithm.old.tex <==
\begin{algorithm}[H]
\caption{Backdoor purification process of \sys.}
\label{alg:1}
\KwIn{Backdoor model $M_{\tilde{\theta}}$, Damping factor $d$, maximum iteration $T$, convergence threshold $\epsilon$  }
\KwResult{Purified model $M_{\text{pf}}$, Evidence $E$}

\SetKwFunction{FMain}{ObtainEvidence}
\SetKwProg{Fn}{Procedure}{:}{\KwRet}
\Fn{\FMain{$M_{\text{bd}}, \text{target}$}}{
    \tcp{Hyperparameters for TextRank} 
    \BlankLine
    \If{Judgment evidence available ($E_{\text{target}}$)}{
        $E \leftarrow$ Modify $E_{\text{target}}$ based on predictions of $M_{\text{bd}}$ using API model\;
    }
    \Else{
        \tcp{Step 1: Construct word graph for TextRank}
        $\text{words} \leftarrow \text{Tokenize}(\text{target})$\;
        $G \leftarrow \text{CreateGraph}(\text{words})$\;
        
        \tcp{Step 2: Initialize node weights}
        \ForEach{$V_i \in G.\text{nodes}$}{
            $W(V_i) \leftarrow 1.0$\;
        }
        
        \tcp{Step 3: Iteratively update weights until convergence}
        \For{$\text{iter} = 1$ \KwTo $\text{max\_iter}$}{
            $W_{\text{prev}} \leftarrow W$\;
            \ForEach{$V_i \in G.\text{nodes}$}{
                $W(V_i) \leftarrow (1 - d) + d \times \sum_{V_j \in \text{In}(V_i)} \frac{W(V_j)}{L(V_j)}$\;
            }
            $\Delta \leftarrow \sum_{V_i \in G.\text{nodes}} |W(V_i) - W_{\text{prev}}(V_i)|$\;
            \If{$\Delta < \epsilon$}{
                \textbf{break}\;
            }
        }
        
        \tcp{Step 4: Determine keywords and the number of evidence pieces}
        $\text{sorted\_words} \leftarrow \text{SortByWeight}(G.\text{nodes})$\;
        $n \leftarrow |\text{sorted\_words}|$\;
        
        \tcp{Step 5: Generate $n$ pieces of evidence based on TextRank result}
        $E \leftarrow \text{GenerateEvidence}(n + \text{sorted\_words})$\;
    }
    \textbf{return} $E$\;
}
\BlankLine
\SetKwFunction{FMain}{MergeModels}
\SetKwProg{Fn}{Procedure}{:}{\KwRet}
\Fn{\FMain{$M_{\text{bd}},  t$}}{
    Init $M_{\text{pf}} \leftarrow \emptyset$ \tcp{$M_{\text{pf}}$: Purified model parameters}
    \tcp{Train $M_{\text{cf}}$ using a benign low-rank matrix update}
    $M_{\text{cf}} \leftarrow  W_0 x + \Delta W x$ \tcp{$W_0$: Initial parameters, $\Delta W$: Small rank update to the weights}
    \BlankLine
    \For{$M_i \in M_{\text{bd}}$}{
      
      $W_{\text{cf}} \leftarrow M_{\text{cf}}$
      \tcp{Parameters of conflict model}  
      
      \tcp{Merge the parameters using the provided linear combination}
      
      
      $W_{\text{merge}} \leftarrow t \cdot W_{\text{bd}} + (1-t) \cdot W_{\text{cf}}$
      
      $M^* \leftarrow W_{\text{merge}}$
      
      $C(M^*)$ \tcp{$C$: Internal conflicts within the model using $M^*$}
      
      $M_{\text{pf}} \cup= {M^*}$
      \BlankLine
    }
    \textbf{return} $M_{\text{pf}}$
}

\end{algorithm}

==> tab/discussion-percentage-of-clean-data.tex <==
\begin{table}[tt]

	\caption{Impact of the percentage of the required training samples on defense performance.}
	\label{tab:percentage}
	\centering
	%\scriptsize
	\setlength\tabcolsep{1.5pt}
         \footnotesize
         %\setlength\tabcolsep{9pt}
	\begin{tabular}{c|ccccccccccc}
		\toprule
            %Dataset&
            \multirow{2}{*}{\shortstack{Precentage}}&\multicolumn{2}{c}{\color{black}LLaMA}&\multicolumn{2}{c}{\color{black}GPT-XL}&\multicolumn{2}{c}{\color{black}LLaMA-2}&\multicolumn{2}{c}{\color{black}GPT-J}\\
            &CBA&DTBA&CBA&DTBA&CBA&DTBA&CBA&DTBA\\
      \midrule
          %\multirow{18}{*}{\shortstack{CIFAR-100}}&
          5\%&2.17\%&32.0\%&32.27\%&38.0\%&26.41\%&22.0\%&48.58\%&23.0\%\\
          10\%&1.18\%&10.5\%&15.34\%&32.0\%&11.27\%&9.0\%&11.16\%&3.0\%\\
          15\%&2.88\%&10.0\%&5.86\%&6.0\%&10.29\%&8.0\%&24.00\%&4.5\%\\
          20\%&0.76\%&18.0\%&4.91\%&3.0\%&9.86\%&10.0\%&22.46\%&1.0\%\\
          25\%&1.02\%&6.5\%&4.32\%&8.0\%&8.81\%&8.0\%&17.43\%&2.5\%\\
          30\%&0.71\%&9.0\%&3.91\%&12.0\%&9.73\%&7.0\%&9.12\%&1.5\%\\
          40\%&0.76\%&6.0\%&4.06\%&1.0\%&7.25\%&6.5\%&5.56\%&0.5\%\\
          50\%&1.02\%&3.0\%&3.43\%&1.0\%&9.26\%&5.0\%&8.93\%&0.0\%\\
          100\%&0.86\%&1.0\%&3.55\%&0.0\%&6.33\%&3.0\%&6.37\%&0.0\%\\
        \bottomrule
	\end{tabular}
 %\vspace{-0.4cm}
  
\end{table}
